Tabular Few-Shot Generalization Across Heterogeneous Feature Spaces

Despite the prevalence of tabular datasets, few-shot learning remains under-explored within this domain. Existing few-shot methods are not directly applicable to tabular datasets due to varying column relationships, meanings, and permutational invariance. To address these challenges, we propose FLAT-a novel approach to tabular few-shot learning, encompassing knowledge sharing between datasets with heterogeneous feature spaces. Utilizing an encoder inspired by Dataset2Vec, FLAT learns low-dimensional embeddings of datasets and their individual columns, which facilitate knowledge transfer and generalization to previously unseen datasets. A decoder network parametrizes the predictive target network, implemented as a Graph Attention Network, to accommodate the heterogeneous nature of tabular datasets. Experiments on a diverse collection of 118 UCI datasets demonstrate FLAT's successful generalization to new tabular datasets and a considerable improvement over the baselines.

==> figures/medical_results_bydataset.tex <==
\begin{tabular}{p{2.8cm}cccccccccccc}
\toprule
\multicolumn{1}{r}{} & \multicolumn{9}{c}{\textbf{model}} &\\
\cmidrule{2-12}
\textbf{test dataset}           & \rot{\textbf{TabNet}} & \rot{\textbf{TabPFN}} & \rot{\textbf{RForest}} & \rot{\textbf{LR}} & \rot{\textbf{CatBoost}} & \rot{\textbf{SVC}}  & \rot{\textbf{FTT}}  & \rot{\textbf{KNN}} & \rot{\textbf{STUNT}} & \rot{\textbf{Iwata}} & \rot{\textbf{FLAT}} \\
\midrule
thyroid & 52.4 & 58.4 & 63.9 & 61.4 & 69.4 & 61.6 & 60.5 & 56.9 & 58.5 & 57.3 & 59.7 \\
ilpd-indian-liver & 51.1 & 50.0 & 51.0 & 50.8 & 51.6 & 51.7 & 52.7 & 51.8 & 53.5 & 54.8 & 52.0 \\
acute-inflammation & 61.4 & 72.6 & 75.1 & 75.4 & 74.3 & 76.0 & 77.4 & 79.6 & 76.5 & 61.1 & 76.9 \\
heart-cleveland & 53.1 & 64.3 & 66.7 & 67.6 & 66.5 & 70.6 & 68.7 & 71.0 & 70.3 & 77.5 & 74.9 \\
heart-va & 48.7 & 50.8 & 50.4 & 49.9 & 49.5 & 50.7 & 50.4 & 49.7 & 50.3 & 47.2 & 48.5 \\
post-operative & 53.0 & 50.7 & 50.6 & 49.9 & 49.0 & 49.7 & 48.5 & 48.0 & 48.8 & 51.1 & 51.0 \\
breast-cancer-wisc-diag & 51.6 & 76.3 & 76.4 & 80.1 & 81.0 & 83.4 & 82.1 & 81.8 & 82.9 & 87.4 & 85.5 \\
acute-nephritis & 60.0 & 75.9 & 81.6 & 80.7 & 83.2 & 83.7 & 81.9 & 88.6 & 82.9 & 91.1 & 89.3 \\
horse-colic & 50.6 & 58.0 & 61.3 & 62.7 & 63.3 & 65.4 & 62.3 & 62.7 & 64.8 & 60.5 & 63.9 \\
blood & 51.5 & 57.1 & 56.5 & 55.5 & 56.3 & 54.9 & 58.2 & 57.0 & 55.7 & 57.1 & 56.8 \\
heart-switzerland & 48.8 & 51.2 & 52.8 & 52.2 & 54.5 & 53.1 & 51.7 & 52.6 & 52.6 & 54.6 & 53.3 \\
lymphography & 49.4 & 57.3 & 60.1 & 59.4 & 62.3 & 62.5 & 64.1 & 65.0 & 60.3 & 67.0 & 65.8 \\
breast-cancer-wisc-prog & 50.9 & 52.7 & 51.4 & 52.3 & 51.2 & 52.3 & 52.5 & 50.2 & 53.4 & 51.8 & 52.3 \\
heart-hungarian & 60.1 & 63.9 & 66.5 & 67.7 & 68.5 & 69.0 & 70.3 & 71.2 & 71.9 & 75.7 & 75.0 \\
breast-cancer & 52.9 & 53.0 & 54.7 & 51.5 & 53.7 & 52.1 & 54.0 & 53.5 & 53.6 & 55.7 & 55.3 \\
statlog-heart & 50.7 & 61.4 & 66.8 & 67.6 & 66.2 & 70.2 & 69.8 & 70.6 & 69.9 & 77.1 & 77.0 \\
breast-cancer-wisc & 53.1 & 91.2 & 89.4 & 92.0 & 92.3 & 92.9 & 92.0 & 93.0 & 94.2 & 95.6 & 95.6 \\
echocardiogram & 53.0 & 56.5 & 58.2 & 59.8 & 58.7 & 60.1 & 62.6 & 62.1 & 62.3 & 68.5 & 68.5 \\
hepatitis & 49.9 & 58.1 & 61.2 & 61.1 & 61.6 & 62.3 & 61.9 & 64.0 & 62.1 & 64.5 & 64.5 \\
dermatology & 53.2 & 78.6 & 79.9 & 83.9 & 84.1 & 89.8 & 86.5 & 92.3 & 85.5 & 93.8 & 93.9 \\
mammographic & 57.7 & 66.2 & 68.0 & 68.0 & 69.1 & 67.0 & 70.7 & 70.4 & 74.1 & 79.0 & 79.3 \\
primary-tumor & 53.3 & 58.2 & 61.4 & 61.6 & 63.5 & 62.5 & 63.4 & 61.8 & 62.5 & 65.5 & 65.8 \\
cardiotocography & 53.3 & 59.6 & 60.0 & 63.0 & 60.5 & 65.6 & 62.7 & 64.4 & 64.4 & 67.8 & 68.4 \\
parkinsons & 51.5 & 64.6 & 66.3 & 68.1 & 66.3 & 68.2 & 68.0 & 68.2 & 69.4 & 70.9 & 71.6 \\
vertebral-column & 57.7 & 62.2 & 60.5 & 64.2 & 61.8 & 62.5 & 64.2 & 62.3 & 65.3 & 65.4 & 66.9 \\
breast-tissue & 56.5 & 83.9 & 83.6 & 87.6 & 85.1 & 87.5 & 89.2 & 88.2 & 87.0 & 89.4 & 91.0 \\
spectf & 48.6 & 65.8 & 66.1 & 67.0 & 68.7 & 68.9 & 68.7 & 66.9 & 71.1 & 73.0 & 76.0 \\
arrhythmia & 51.7 & —* & 54.1 & 54.4 & 55.3 & 55.0 & 55.1 & 54.7 & 55.4 & 54.4 & 58.5 \\
spect & 54.2 & 51.8 & 54.7 & 54.3 & 54.7 & 53.9 & 54.4 & 55.1 & 55.5 & 51.6 & 59.5 \\
\midrule
\textbf{total average} &53.1 &62.5 &63.8  &64.5 &64.9 &65.6 &65.7 &66.0  &66.0 &67.8 &\textbf{68.9} \\
\bottomrule
\end{tabular}



==> figures/medical_results_ranks.tex <==
\begin{tabular}{rccccc}
\toprule
\multicolumn{1}{l}{} & \multicolumn{4}{c}{$N^{meta}$}    \\
\midrule
\textbf{model}       & \multicolumn{1}{c}{1*}         & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{15} \\
\midrule
LR & - & 6.57 & 7.17 & 5.34 & 4.38 \\
KNN & - & 3.64 & 5.31 & 6.43 & 7.62 \\
SVC & - & 5.16 & 5.16 & 5.69 & 6.00 \\
RForest & - & 8.53 & 7.55 & 6.03 & 5.29 \\
CatBoost & - & 6.34 & 6.40 & 6.72 & 6.38 \\
TabNet & - & 10.22 & 10.21 & 10.28 & 10.50 \\
FTT & - & 5.17 & 5.07 & 6.02 & 5.57 \\
STUNT & - & 4.91 & 4.53 & 4.6 & 4.91 \\
TabPFN & 2.79 & 9.16 & 8.62 & 7.48 & 6.05 \\
Iwata & 1.72 & 3.26 & 3.43 & 4.50 & 5.09 \\
FLAT & \textbf{1.47} & \textbf{2.97} & \textbf{2.47} & \textbf{2.78} & \textbf{4.03} \\
\bottomrule
\end{tabular}

